A Comparison of Natural Language Understanding Platforms for Chatbots in Software Engineering

Chatbots are envisioned to dramatically change the future of Software Engineering, allowing practitioners to chat and inquire about their software projects and interact with different services using natural language. At the heart of every chatbot is a Natural Language Understanding (NLU) component that enables the chatbot to understand natural language input. Recently, many NLU platforms were provided to serve as an off-the-shelf NLU component for chatbots, however, selecting the best NLU for Software Engineering chatbots remains an open challenge. Therefore, in this paper, we evaluate four of the most commonly used NLUs, namely IBM Watson, Google Dialogflow, Rasa, and Microsoft LUIS to shed light on which NLU should be used in Software Engineering based chatbots. Specifically, we examine the NLUs' performance in classifying intents, confidence scores stability, and extracting entities. To evaluate the NLUs, we use two datasets that reflect two common tasks performed by Software Engineering practitioners, 1) the task of chatting with the chatbot to ask questions about software repositories 2) the task of asking development questions on Q&A forums (e.g., Stack Overflow). According to our findings, IBM Watson is the best performing NLU when considering the three aspects (intents classification, confidence scores, and entity extraction). However, the results from each individual aspect show that, in intents classification, IBM Watson performs the best with an F1-measure > 84%, but in confidence scores, Rasa comes on top with a median confidence score higher than 0.91. Our results also show that all NLUs, except for Dialogflow, generally provide trustable confidence scores. For entity extraction, Microsoft LUIS and IBM Watson outperform other NLUs in the two SE tasks. Our results provide guidance to software engineering practitioners when deciding which NLU to use in their chatbots.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}
In this section, we dive into the evaluation results to gain more insights on the NLUs' confidence score sensibility as well as quantifying their abilities to extract unique and multiple entities. %Also, we examine the techniques that some NLUs used in their classifications. 
Finally, we provide recommendations to chatbot developers and researchers to achieve better intents classification and entity extraction results.

\subsection{Tuning the NLU's Confidence Score Threshold} %\ahmad{Diego, do you think it is good to place this section as the first section in the discussion to be consistent in the flow same order as the results section?[intents confidence scores then entities?] OR to keep the order as is, because we  are discussing the entities much and we need to use the information in the reader's mind as they are fresh [i.e., the last section in the results is about the entity?]}
%\diego{Good point. Perhaps moving it to the beginning of the section would make more sense (following the order (Intent $\to$ Entity))}

\label{sub:sensitivity-score-threshold}

\begin{figure*}[tbh]
	\centering		
	\begin{subfigure}{0.5\textwidth}	
		\centering	
		\includegraphics[width=.9\linewidth]{Figures/Chatbot_CS.pdf}	
		%		\vspace{-0.2in}
		\caption{Repository Task}	
	\end{subfigure}\hfill	
	\begin{subfigure}{0.5\textwidth}		
		\centering	
		\includegraphics[width=.9\linewidth]{Figures/SOF_CS.pdf}	
		%		\vspace{-0.2in}
		\caption{Stack Overflow Task}	
	\end{subfigure}\hfill	
	\caption{Analysis of theshold sensitivity in terms of F$_1$ measure of the NLUs in the Repository and Stack Overflow Tasks. \diego{Figure will be regenerated}}	
	\label{fig:ConfidenceScoresResults}	
\end{figure*}

%\remove{As we discussed in Section \ref{sec:background}, selecting the confidence score threshold is critical for the Chatbot developers.}
Our results in Section~\ref{subsec:nlusConfidenceScoresResults} show that the distribution of the correctly classified intents vary among NLUs and across tasks. %, also vary across the datasets (i.e., Chatbot and Stack Overflow) for the same NLU as shown in Figure~\ref{fig:ConfidenceScoreResults}. 
While NLUs tend to yield higher score when returning correctly classified intents, defining the appropriate threshold to accept the classified intent or trigger the fallback action is still a challenge for developers. 
%This poses a challenge to chatbot developers to select the most appropriate confidence score threshold, which is crucial for the chatbot performance as discussed in Section~\ref{sec:background}.
%This represents a challenge to chatbot developers because selecting the confidence score threshold is critical for the success of the chatbot as discussed in Section~\ref{sec:background}.
Therefore, to help developers in selecting an appropriate threshold for their chatbots, we examine the impact of different thresholds on the NLU's performance for intents classification. 

Figure \ref{fig:ConfidenceScoresResults} shows the NLUs' F1 measures at different confidence score thresholds. 
We find that Rasa is the most robust (less sensitive) NLU, performing slight better when the threshold is more restrictive (0.5 and 0.6) as opposed to other NLUs.
In general, our results show that the ideal threshold for IBM Watson and Dialogflow is 0.3 for both tasks, which exactly matches the default threshold for Dialogflow.
% hence, developers may not need to further tune this parameter on such NLUs. 
LUIS performance varies considerably in the Repository task , showing its best performance with the threshold of 0.1, but following closely the performance of other NLUs in the Stack Overflow data.
Therefore, we recommend for SE tasks a threshold of 0.3 for Dialogflow, IBM Watson and LUIS and a higher threshold for Rasa (e.g., 0.5, 0.6). 
However, chatbot developers should be able assess the best threshold for their dataset using similar analysis. 


%On the other hand, LUIS has low performance regardless of the threshold for the Chatbot corpus due to the large number of misclassified intents. \ahmad{Maybe we need to have an implications or closing sentence, as ``We are planing in the future to examine those thresholds using more datasets from the SE domain.''}




\subsection{Unique Entities}
%As seen in evaluation results for the Stack Overflow corpus, the unique entities affect the extraction performance of the NLUs. To better understand the NLUs ability to extract unique entities (i.e., entities that the NLU has not been trained on), we select the queries that include only unique entities from the Stack Overflow corpus. In other words, we remove queries that have no entities and those with one or more non unique entities. This is to ensure that our evaluation is not affected by the extraction of non unique entities, as all of the NLUs (except for Rasa) in our evaluation are closed source code. As a result, we have 58 queries that include 75 unique entities which are distributed as shown in Table \ref{table:Multiple_Unique_Entity_Distribution}. We use the same criteria mentioned in Section \ref{subsec:entityExtractionResult} to calculate the Precision, Recall, and F1-measure to evaluate the extraction of unique entities. 
%
%
%The evaluation results for all NLUs in unique entities extraction are shown in Table \ref{NLU_Extract_Unique_Entities}. Also, our analysis of these results shows that the NLUs depend on the entities similarity to extract the unique entities, as discussed in section \ref{subsec:entityExtractionResult}. This gives the NLUs the ability to extract entities that they have not been trained on before, although the entity type is not always extracted correctly. 


%Another interesting finding is that the incorrectly extracted entities are related to multi-worded entities. An entity is considered to be multi-worded if its value contains more than one word (e.g., `SAP crystal reports' is a single entity of type `Fram'). In the Stack Overflow corpus, the multi-worded entities are always unique entities (except for two; `Internet Explorer' and `WebSphere 8.5.5'). In the selected queries for the evaluation of unique entities, 22.7\% of all entities are unique multi-worded entities. Surprisingly, none of the NLUs extract any unique multi-worded entity correctly except for IBM Watson, which only extracts 17.7\% of those entities. 
%Also, we find that the NLUs return one of the words in the multi-worded entity as a separate entity on its own, because the NLU is trained on that separate entity. For example, the multi-worded entity `Python NameError' with an `API' type is extracted by all NLUs as the entity `Python' of type `PL'. This overlapping between the multi-worded entities and other entities misleads the NLUs. This is mostly present in IBM Watson and Dialogflow, as they incorrectly extract all the overlapping multi-worded entities. Instead, both NLUs extract a single word from the multi-worded entity as a standalone entity.
%%(e.g., from `Java Web-Start' both NLUs only extract `Java').
%
%
%This clearly shows that the unique multi-worded entities should be given a special care when added, especially, if one of their words is a separate entity. Also, the results show the need of tools/techniques from the research community to help bots developers to overcome the aforementioned issue. We plan to evaluate the NLUs using non unique multi-worded entities in the future since all NLUs extract all such entities (`Internet Explorer' and `WebSphere 8.5.5') that exist in our corpus.  
%
%\ahmad{====================}
%The performance of the NLUs in extracting entities from the Stack Overflow task was affected by unique entities, as shown in Section \ref{subsec:entityExtractionResult}. 
%As the name suggests, unique entities appear just once in the task  (once in the dataset), thus, NLUs have to predict their occurrence without prior training.
%To better understand the NLUs' ability to extract unique entities, we investigate the results from the Stack Overflow task, examining queries containing only unique entities. 
%This is to ensure that our evaluation is not affected by the extraction of non-unique entities. 
%We find 58 queries that fit this evaluation, and they include a total of 75 unique entities that are distributed as shown in Table \ref{table:Multiple_Unique_Entity_Distribution}. 
%Similarly to the evaluation conducted in Section~\ref{subsec:entityExtractionResult}, we calculate the precision, recall, and F1-measure of the NLUs when extracting unique entities.
%
%
%Table~\ref{NLU_Extract_Unique_Entities} presents the unique entities extraction results of all NLUs. 
%We observe that IBM Watson (31.6\% F1 measure) has the best performance by a large margin, followed by LUIS (7.7\%) and Rasa (2.1\%). 
%Dialogflow failed to extract any unique entity from the set of 58 queries.
%Upon closer examination in the results, we find that the reason behind the incorrect extraction of unique entities can be explained by two reasons.
%First, the NLUs depend on the entities similarity to extract the unique entities and sometimes the syntax similarity may drive the NLUs to recognize the wrong entity.
%For example, the query ``Recieving 0.0 when multiplying two doubles in an array" had `Receiving 0.0' wrongly extracted as an entity of type Framework (`Fram'), because it is syntatically similar to Framework entities such as `Spring 4.0.2' and `CodeIgniter 2.0.3'. 
%Second, some of the incorrectly extracted entities are related to multi-worded entities (e.g., `SAP crystal reports' is a single entity of type `Fram'). 
%In the Stack Overflow task, 22.7\% of all unique entities are multi-worded. 
%With the exception of a few examples (`Internet Explorer' and `WebSphere 8.5.5'), almost all multi-worded entities are unique in the Stack Overflow task.
%Evaluating the performance only with queries with multi-worded entities, we found that IBM Watson obtained a F1-measure of 17.7\%, whereas the other NLUs are unable to extract any unique multi-worded entity correctly (F1-measure of 0\%). 
%This happens because the NLUs extract one of the words in the multi-worded entity as a separate entity on its own, given the NLUs are trained on such separate entities. 
%For example, the multi-worded entity `Python NameError' with an `API' type is extracted by all NLUs as the entity `Python' of type `PL'. This overlapping between the multi-worded entities and other entities misleads the NLUs. And, it is mostly present in IBM Watson and Dialogflow, as they incorrectly extract all the overlapping multi-worded entities.

%This clearly shows that the unique multi-worded entities should be given special care when added, especially, if one of their words is a separate entity. Also, the results show the need for tools/techniques from the research community to help the bot developers to overcome the aforementioned issue. We plan to evaluate the NLUs using non-unique multi-worded entities in the future since all NLUs extract all such entities (`Internet Explorer' and `WebSphere 8.5.5') that exist in our task.

The performance of the NLUs in extracting entities from the Stack Overflow task was affected by unique entities as shown in Section~\ref{subsec:entityExtractionResult}. As the name suggests, unique entities appear just once in the dataset for the Stack Overflow task, thus, NLUs have to predict their occurrence without prior training on them. It is important to note that there are no unique entities when evaluating the NLUs using the list feature because the NLUs have been trained on all entities that exist in the Repository task.
To better understand the NLUs' ability in the extraction of unique entities, we investigate the results from the Stack Overflow task, examining the NLU performance on queries containing only unique entities.
Hence, queries containing any non-unique entity were excluded from this investigation.  
%This is to ensure that our evaluation is not affected by the extraction of non-unique entities. 
We find 58 queries that fit our criteria, and they include a total of 75 unique entities that are distributed as shown in Table~\ref{table:Multiple_Unique_Entity_Distribution}. 
Similarly to the evaluation conducted in Section~\ref{subsec:entityExtractionResult}, we calculate the precision, recall, and F1-measure of the NLUs when extracting unique entities.


Table~\ref{NLU_Extract_Unique_Entities} presents the NLUs' performance of in extracting unique entities. We find that IBM Watson (31.6\% F1-measure) has the best performance by a large margin, followed by LUIS and Rasa. Dialogflow failed to extract any unique entity from the set of 58 queries. We examine the unique entities extraction results and find two reasons that impact the NLUs' performance. First, the NLUs depend on the entities syntax similarity to recognize the entities in the queries of the testing set. For example, the query ``Receiving 0.0 when multiplying two doubles in an array" had `Receiving 0.0' wrongly extracted as an entity of type Framework (`Framework'), because it is syntactically similar to Framework entities such as `Spring 4.0.2' and `CodeIgniter 2.0.3'. 
Second, we find that the NLUs extract one of the words in the multi-worded entity (e.g., `SAP crystal reports' is a single entity of type `Framework') as a separate entity on its own, given the NLUs are trained on such separate entities. For example, the multi-worded entity `Python NameError' with an `API' type is extracted by all NLUs as the entity `Python' of type `ProgLanguage'. With the exception of a few examples (`Internet Explorer' and `WebSphere 8.5.5'), almost all multi-worded entities are unique in the Stack Overflow task. 
%\diego{I think we should drop the multi-worded entities (next sentence). We don't even show this in a table...}
Evaluating the performance only with queries with multi-worded entities, we found that IBM Watson obtained a F1-measure of 17.7\%, whereas the other NLUs are unable to extract any unique multi-worded entity correctly. This clearly shows that the unique multi-worded entities should be given special care when added.
Hence, these results motivate the need for tools/techniques from the research community to extract the unique entities. Also, we encourage the chatbot developers to give special attention to unique entities by training the NLU on more examples by including those entities.
 
%help the chatbot developers to overcome the aforementioned issue


%Also, the results show the need for tools/techniques from the research community to help the bot developers to overcome the aforementioned issue. We plan to evaluate the NLUs using non-unique multi-worded entities in the future since all NLUs extract all such entities (`Internet Explorer' and `WebSphere 8.5.5') that exist in our task.




\begin{table}[]
	\centering
	\caption{Distribution of Unique and Multiple Entities By Entity Type}
	\label{table:Multiple_Unique_Entity_Distribution}
	\begin{tabular}{lrr}
		\toprule
		\textbf{Entity} & \textbf{Unique} & \textbf{Multiple} \\ 
		
		\textbf{Type}		& \textbf{Entities}					&\textbf{Entities}									\\
		
		\midrule
		ProgLanguage & 1 & 45 \\
		Framework & 36 & 18 \\
		Standard & 5 & 6 \\
		API & 32 & 15 \\
		Platform & 1 & 4 \\ 
		\bottomrule
	\end{tabular}
\end{table}

\begin{table}[]
	\centering
	\caption{NLUs Accuracy in Extracting Unique Entities in the Stack Overflow Task}
	\label{NLU_Extract_Unique_Entities}
	\begin{tabular}{lrrr}
		\toprule
		\textbf{NLU} & \textbf{Precision} & \textbf{Recall} & \textbf{F1-Measure} \\ 
		\midrule
		IBM Watson & 51.4\% & 28\% & 31.6\% \\
		Dialogflow & 0.0\% & 0.0\% & 0.0\% \\
		Rasa & 12\% &1.3\% & 2.1\% \\
		LUIS & 25.3\% & 5.3\% & 7.7\%\\ 
		\bottomrule
	\end{tabular}
\end{table}
\iffalse
\diego{Where are these results shown?? I am very confused here.}
\diego{Ahmad, as discussed: try to simplify these two paragraphs and incorporate the essential into the last paragrap. Right now, it is quite confusing why yet another analysis is done here.}
To gain more insights on why the multi-worded entities are not correctly extracted by the NLUs, we deep-dive into the results. We find that the NLUs return one of the words in the multi-worded entity as a separate entity on its own, because the NLU is trained on that separate entity. For example, the multi-worded entity `Python NameError' with an `API' type is extracted by all NLUs as the entity `Python' of type `ProgLanguage'. This overlapping between the multi-worded entities and other entities misleads the NLUs. And, it is mostly present in IBM Watson and Dialogflow, as they incorrectly extract all the overlapping multi-worded entities.
% Instead, both NLUs extract a single word from the multi-worded entity as a standalone entity.
\fi



\subsection{Multiple Entities}


%In the Stack Overflow task, we notice that some queries have more than one entity, e.g., ``PHP script not receiving post data'' which has the entities `PHP' of type `PL' and `Post' of type `API'. 
%Therefore, we want to investigate the NLUs' ability to extract multiple entities from the posed queries. To do that, we examine the results from the queries that have more than one entity and do not have any unique entities in them. 
%This is to avoid any external factors (if any) that might impact the analysis results. 
%In total, we find 42 queries that satisfy our criteria and they contain 88 entities (31.3\% of entities in the task) distributed as shown in Table \ref{table:Multiple_Unique_Entity_Distribution}. 
%
%The evaluation results for all the NLUs in extracting multiple entities are shown in Table \ref{table:Multiple_entity_extraction_results}. Dialogflow outperforms other NLUs in extracting multiple entities with an F1-measure of 83.5\%, followed by IBM Watson (80.3\%), Rasa (73.6\%) and LUIS (66.5\%). 
%The results differ slightly from the general entity extraction with Dialogflow coming up in the first place.
%Overall, we found that all evaluated NLUs perform reasonably well in queries with multiple entities, with higher performance than the general evaluation, showing that they are apt to be used well in context where multiple parameters are needed to answer a query.

The chatbots in the SE domain most likely receive queries that have more than one entity. For example, `PHP script not receiving post data'' which has the entities `PHP' of type `ProgLanguage' and `Post' of type `API'. Consequently, we want to investigate the NLUs' ability to extract multiple entities from the posed queries. To do that, we examine the results from the queries that have more than one entity and do not have any unique entities in them. This is to avoid any external factors (if any) that might impact the analysis results. In total, we find 42 queries that satisfy our criteria and they contain 88 entities (31.3\% of entities in the task) distributed as shown in Table \ref{table:Multiple_Unique_Entity_Distribution}. These queries belong to Stack Overflow task as there are no queries with multiple entities in the Repository task.

Table~\ref{table:Multiple_entity_extraction_results} shows the evaluation results for all the NLUs in extracting multiple entities. The results differ slightly from the general entity extraction in Section~\ref{subsec:entityExtractionResult} with Dialogflow coming up in the first place in extracting multiple entities with an F1-measure of 83.5\%, followed by IBM Watson (80.3\%), Rasa (73.6\%) and LUIS (66.5\%). Overall, we found that all evaluated NLUs perform reasonably well in queries with multiple entities, with higher performance than the general evaluation, showing that they are apt to be used well in context where multiple parameters are needed to answer a query.

\begin{table}[]
	\centering
	\caption{NLUs Accuracy in Extracting Multiple Entities in the Stack Overflow Task}
	\label{table:Multiple_entity_extraction_results}
	\begin{tabular}{lrrr}
		\toprule
		\textbf{NLU} & \textbf{Precision} & \textbf{Recall} & \textbf{F1 Measure} \\ 
		\midrule
		IBM Watson & 95.2\% & 79.6\% & 80.3\% \\
		Dialogflow & 95.0\% & 84.1\% & 83.5\% \\
		Rasa & 90.9\% & 70.5\% & 73.6\% \\
		LUIS & 87.5\% & 61.4\% & 66.5\% \\ 
		\bottomrule
	\end{tabular}
\end{table}


%\subsection{Combining NLUs for Better Performance}
%
%In this section, we explore the possibility of creating an ensemble NLU, containing all NLUs evaluated in this study.
%Ensemble models combine two or more models to obtain more predictive power, by increasing the stability of models and reducing the variance in the models' prediction. 
%We combine all NLUs using a variance of bootstrap aggregating~\diego{Ref}, where each NLU votes with equal weights for the intent classification.
%If no majority is obtained, we use the highest confidence score of the voters to determine the classified intent.
%With this model, we manage to obtain a boost in performance compared to IBM Watson in the Chatbot corpus with F1-measure of 93.63 (+10.6\%) but scored 2nd place in the Stack Overflow corpus with F1-measure of 80.32 (-4.7\%).
%Overall, this performance gain may not justify the costs of maintaining multiple NLUs, but this ensemble model can be used by researchers particularly in tasks where the most optimal performance is crucial, such as labeling datasets. 




%for labeling datasets with a small training sample.

%\diego{Finish this section}
%We did the voting for the NLUs and we take the intents that has the major votes.
%In case that there is no consensus (each NLU has it's own classification or 2 NLUs agreed on something and the other 2 agreed on something else) we look into the confidence scores of those NLUs and we took the intent classification of the higher confidence scores.
%Results (weighted F1):
%\begin{itemize}
%	\item Chatbot - voting: 91.77
%	\item Chatbot - confidence scores: 93.63
%	\item Stack Overflow - voting: 79.52
%	\item Stack Overflow - confidence score: 80.32
%\end{itemize}



\iffalse

\subsection{Different Context}
%Prior work shows that the NLU performance varies between different domains. For example, Dialogflow outperformed other NLUs in identifying intents and entities using a corpus from student admission domain \cite{gregori_2017GIT}. On the other hand, LUIS achieved the best in classifying intents and extracting entities in public transport connections and StackExchange corpora \cite{braun_SIGDIAL2017}. However, when we use two datasets from the same domain (i.e., SE) to evaluate the NLUs, our results show that the performance of each NLU varies between the two corpora. Although, the ranking order of all NLUs remains the same in both datasets with regards to intents classification. The reason for the difference in performance between the datasets is mainly due to the nature of the queries in each corpus. One fundamental difference between the two datasets is that in the Chatbot corpus, users of the bot know that they are posing questions to a bot. Therefore, they tend to make their questions more understandable to the bot \cite{braun_SIGDIAL2017}. On the other hand, in the Stack Overflow corpus, users expect other users to read the titles and bodies of their questions. Thus, making the questions' titles less clear. This can be better seen in the disagreement (34\%) between the second author and the recruited Ph.D. student who read only the titles during the labelling stage.
%
%On the other hand, we notice that the entities extraction results and ranking order of the NLUs are affected by the feature. For example, LUIS achieves the best performance in extracting entities from the Chatbot corpus using the list feature, but it comes last in the Stack Overflow corpus where the list feature is not used. Also, IBM Watson outperforms other NLUs in extracting entities from the Stack Overflow corpus but it has a poor performance in the Chatbot corpus when using the list feature. Another reason for this difference can be related to using different datasets. However, we plan to validate the NLUs performance in extracting entities by comparing the list and the prediction features using the same corpus in the future. 
%
%In general, the results show that the NLUs performance in extracting intents and entities varies not only between different domains, but also between different corpora within the same domain \ahmad{as shown in the previous study \emad{add the citation}}. Therefore, the bots developers can depend on different NLUs at the same time to get optimal results. For example, they can use one NLU (e.g., IBM Watson) to classify the intents and another one (e.g., LUIS) for entities extraction in their bot implementation.
%
%\ahmad{============}
\diego{I am not sure about this section. We already start the paper by saying that different NLUs seem to perform best on different scenarios. I don't see what we are bringing to the table with this section.}
Prior work shows that the NLU performance varies between different domains. For example, Dialogflow outperformed other NLUs in identifying intents and entities using a corpus from student admission domain \cite{gregori_2017GIT}. On the other hand, LUIS achieved the best in classifying intents and extracting entities in public transport connections and Stack Exchange corpora \cite{braun_SIGDIAL2017}. In our study, the majority of the differences between the intents classification and entity extraction results among the NLUs are not statistically significant. Consequently, it is difficult to state that one NLU outperforms all the others. Overall, Rasa tends to be the most suitable platform for Chatbots that operate in the context of SE. This is because Rasa is the most confident in its classification results and has a similar performance to other NLUs in intents classification and entity extraction (except for unique entities). Moreover, it is less sensitive towards the tuning of the confidence score threshold compared to other NLUs. Our results differ from other studies that evaluate NLUs in other domains. This is mainly because SE is a specialized domain with words that have different contexts, such as file names and special multi-worded entities (e.g., software versions [spring 4.0.2]).
%than other domains (e.g., insurance domain)\khaled{I feel that a stronger argument can come from this: The SE domain has words such as file names, commit hashes, }\ahmad{Can we merge it with the previous sentence?}

%Moreover, our results show that the performance of each NLU varies between the two corpora, although the ranking of the NLUs in intents classification remains the same between the datasets., the performance deffirence in entities extraction is more visible. The reason behind this is mainly due to the nature of the queries in each corpus. One fundamental difference between the two datasets is that in the Chatbot corpus, users of the bot know that they are posing questions to a bot. Therefore, they tend to make their questions clearer and more understandable to the bot \cite{braun_SIGDIAL2017}. On the other hand, in the Stack Overflow, users expect other users to read the titles and bodies of their questions and thus, making the questions' titles less clear. We believe that our results show a need for more studies that evaluate the NLUs using different datasets in the SE domain, such as code review data. 

Moreover, our results show that the performance of each NLU in intents classification varies between the two corpora. The reason behind this is mainly due to the nature of the queries in each corpus. One fundamental difference between the two datasets is that in the Chatbot corpus, users of the bot know that they are posing questions to a bot. Therefore, they tend to make their questions clearer and more understandable when communicating with the bot \cite{braun_SIGDIAL2017}. On the other hand, in the Stack Overflow, users expect other users to read the titles and bodies of their questions and thus, making the questions' titles less clear. We believe that our results show a need for more studies that evaluate the NLUs using different datasets in the SE domain, such as code review data.

%WE DID NOT ADD THE PERFORMACE OF THE ENTITIES EXTRACTION BECAUSE EACH DATA SET REQUIRED DIFFERENT NLU'S FEATURE TO EXTRACT IT, CHATBOT USED LIST FEATURE WHILE SOF USED PREDICITION FEATURE. HOWEVER, WE CAN NOT COMPARE APPLES WITH ORANGES.
\fi

\iffalse

\subsection{NLU in Depth} 

\ahmad{I highlighted the text that we can use at the end of section 3.1. However, I am not sure if it is a good fit in section 3.1, what do you think Diego?}
\diego{I am not so convinced that this section would fit well neither here or there. }

\ahmad{We set ourselves to have a closer look at IBM Watson, Dialogflow, Rasa, and LUIS to have better insights on how those NLUs internally work. Hence, it helps the community to improve the underlying machine learning models used in the classification for the SE domain. We carefully examined the documentation and public forums of all NLUs to understand the underlying machine learning models used in the classification. Also, we reviewed the Rasa source code since it is the only open source NLU in our study. At the end of our investigation, we are able to reveal the used models for IBM Watson and Rasa. Unfortunately, we did not find any information about the classification models of Dialogflow and LUIS in their documentations and forums. We contacted both NLUs' technical support teams through their official channels to inquire about their implementation model. However, we did not get useful replies in both cases, and we received the following response from Dialogflow support team: ``Thank you for showing interest in Dialogflow. But sorry, we cannot disclose any information about our machine learning algorithms and NLU techniques.''}

\textbf{IBM Watson.}
\ahmad{IBM Watson leverages the neural network that is trained on one billion words from Wikipedia \cite{braun_SIGDIAL2017,angara_2018towards,BestChat95:online}. Moreover, IBM Watson uses a technique called ``transfer learning'', that enables developers to harness the training knowledge of a neural network for one task and apply it to another domain. For example, it is used to train the neural network on a task (e.g., text classification) using a very large dataset on one domain (e.g., Wikipedia) and transfer this knowledge to be applied on a similar task with few training examples in a different domain (e.g., software engineering) \cite{Weiss_2016BigDataJournal, Pan_2010TKDE}.} This might justify the reason that IBM Watson extracted more unique entities compared to other NLUs since it has been trained on a huge corpus (i.e., Wikipedia). Moreover, transfer learning allows IBM Watson to learn faster using a small dataset \cite{Weiss_2016BigDataJournal} which we noticed its fast training speed in our experiment compared to the other NLUs. We encourage the SE researchers to investigate the benefits of using transfer learning for the same domain. In other words, train the neural network using different SE datasets such as Stack Overflow and Github, then transfer this knowledge to perform other tasks in the SE domain. 

\textbf{Rasa.} \ahmad{The text for Rasa need to be summerized. I can do that if we agree that the we can fit the text into section 3.1}
One big advantage of using Rasa, besides working on an open-source code, is that it allows Chatbot developers to customize the entire pipeline that better suits their domains. For example, we use the Duckling component in our experiment to extract DateTime entities. Rasa allows developers to easily integrate their custom components in the Rasa pipeline instead of using the pre-existing ones (e.g., Tokenizer). Rasa provides two main predefined pipelines (pretrained\_embeddings\_spacy and supervised\_embeddings) for classification. The pretrained\_embeddings\_spacy is a Spacy pre-trained model that is recommended to be used when the training set has very few examples \cite{ChoosingRasaPipeline_link}. On the other hand, the supervised\_embeddings pipeline uses a neural network in the intent classification and will be customized for the user's domain \cite{ChoosingRasaPipeline_link}. In our study, we use the supervised\_embeddings pipeline in Rasa configuration because our main goal is to examine the NLUs performance when they are customized for the SE domain. On the other hand, Rasa leverages conditional random fields (CRF) to extract entities from the user's queries where it uses different features of the words in the query (e.g., POS tagging). CRF model passes with flying colors in extracting SE entities from Stack Overflow \cite{Ye_2016Saner}. Exploring different features (e.g., sliding window size) to enhance the CRF model requires more investigations to construct a global CRF model for the SE domain.

That said, most of the popular NLUs are closed source (e.g., Dialogflow) where the used pipelines and models are concealed or semi-revealed for public. Therefore, Chatbot developers need to use NLUs as a black-box through their APIs or platforms without tailoring the NLU to their domains. We strongly believe that pipeline customization and integrating third-party libraries to the pipeline that fit the domain would significantly improve the performance of the NLUs (e.g., Duckling library in Rasa). Another major threat of using the NLUs as a black-box is the security of your data. In other words, the NLUs providers might use the data of their users to improve their global machine learning models. At the same time, using those NLUs as an external platform allows developers to focus on the core functionalities of the bot rather than configuring those platforms to work well in a local machine or cloud. Overall, there are many aspects other than the NLU's performance that are involved in the NLU selection for the chatbot implementation such as security and simplicity. The project manager and developers have the final word to make the trade-off decision on which NLU to use in the Chatbot implementation based on the bot's provided functionalities and domain. 

\fi


\subsection{Recommendations}
%Based on our findings, we recommend developers to train the NLU on queries that have different structures (e.g., sentence length) to achieve a higher intents classification accuracy~\cite{multiple17:online}. For NLUs' confidence score, developers should compare the confidence scores of the correctly classified and misclassified intents prior to choosing the cut-off threshold of the bot. And, use other measures (if possible) besides the confidence scores to validate the classified intent by the NLU. For example, if all queries in the training set for a particular intent include a specific entity type, then developers could confirm the classified intent by verifying the existence of an entity of that type in the query. Actually, Dialogflow and IBM Watson use the extracted entities in the intents classifications process~\cite{EntityIntentExtractionDF_link,EntityIntentExtractionIBMWatson_link}. 
%
%On the other hand, the type of entities that the bot expects from the user determines which NLU feature (lookup or prediction features) to use in entities extraction. In case the entities and their synonyms are restricted, the lookup feature is the best choice. Otherwise, the prediction feature is more suitable when the training set does not include all possible entities in the expected queries. For the lookup feature, developers should filter out the common words from the synonym list of the different entities~\cite{RASA_filterCommonWordslink} and include/attach punctuation (e.g., period or question mark) to entities in order to improve their extraction results~\cite{EntityIntentExtractionIBMWatson_link}. However, the NLUs should be trained on more entities at different locations in the queries when using the prediction feature \cite{Goodexam67:online}. Finally, we highly recommend developers to use queries that are posed by real users to train the bot when it is in production. Because it is difficult to include all the possible ways that users might ask the bot, especially when it is deployed for the first time.
%
%
%\ahmad{===========}
%Based on our findings and observations, we provide a set of recommendations to help bot developers and researchers improve the performance of the NLU when operating in the SE domain to increase the satisfaction of the bot users. To achieve a higher intents classification accuracy, we recommend bot developers to train the NLU on queries that have different structures (e.g., sentence length) and position of entities~\cite{multiple17:online}.\\ 
%For the NLUs' confidence score, we suggest that developers compare the confidence scores of the correctly classified and misclassified intents by the used NLU prior to choosing the confidence score threshold value of the bot. And, use other measures (if possible) besides the confidence scores to validate the classified intent by the NLU. For example, if all queries in the training set for a particular intent include a specific entity type, then developers can confirm the classified intent by verifying the existence of an entity of that type in the query. Actually, Dialogflow and IBM Watson use the extracted entities in the intents classifications process~\cite{EntityIntentExtractionDF_link,EntityIntentExtractionIBMWatson_link}.
%
%On the other hand, the type of entities that the bot expects (context of usage) from the user determines whether to use the lookup or prediction feature in entity extraction. In case the entities and their synonyms are restricted, the lookup feature is the best choice. Otherwise, the prediction feature is more suitable when the training set does not include all possible entities in the expected queries. For the lookup feature, developers should filter out the common words from the synonym list of the different entities~\cite{RASA_filterCommonWordslink} and include/attach punctuation (e.g., period or question mark) to entities in order to improve their extraction results~\cite{EntityIntentExtractionIBMWatson_link}. However, the NLUs should be trained on more entities at different locations in the queries when using the prediction feature \cite{Goodexam67:online}. Finally, we highly recommend bot developers to use queries that are asked by real users to train the NLU when their bot is in production. Because it is difficult to include all the possible ways that users might ask the bot, especially when it is deployed for the first time.
%\ahmad{==============}
%\diego{We need to structure this section more like a guideline, with actionable recommendations.}
%Based on our findings and observations, we provide a set of recommendations to help bot developers and researchers improve the performance of the NLU when operating in the SE domain to increase the satisfaction of the bot users. Our results show that the NLUs perform poorly when classifying queries with intents that have a small training set. Therefore, we recommend bot developers to generate more training examples that have different structures (e.g., sentence length) and positions of entities~\cite{multiple17:online} to achieve a higher intents classification accuracy.\\
%
%For the NLUs' confidence score, our findings show that not all NLUs return low confidence scores when misclassifying the user's intent (e.g., Dialogflow). Consequently, we suggest that developers compare the confidence scores of the correctly classified and misclassified intents by the used NLU prior to choosing the confidence score threshold value of the bot. And, use other measures (if possible) besides the confidence scores to validate the classified intent by the NLU. Developers that leverage Dialogflow in their bot implementation are using regular expressions to validate the classified intent by the NLU as discussed in Section \ref{subsec:entityExtractionResult}. Another measure that can be used by bot developers in case of all queries in the training set for a particular intent include a specific entity type is to verify the existence of an entity of that type in the query (e.g., queries of `FixingCommitsForBugTicket' intent has `JiraTicket' entity). Actually, Dialogflow and IBM Watson use the extracted entities in the intents classifications process~\cite{EntityIntentExtractionDF_link,EntityIntentExtractionIBMWatson_link}.
%
%Our results reveal that there is no statistically significant difference in entity extraction results among all NLUs for Chatbot and Stack Overflow corpora using both features. In general, the type of entities that the bot expects (context of usage) from the user determines whether to use the list or prediction feature in entity extraction. In case the entities and their synonyms are restricted, the list feature is the best choice. Otherwise, the prediction feature is more suitable when the training set does not include all possible entities in the expected queries. For the list feature, developers should filter out the common words from the synonym list of the different entities~\cite{RASA_filterCommonWordslink} and include/attach punctuation (e.g., period or question mark) to entities in order to improve their extraction results~\cite{EntityIntentExtractionIBMWatson_link,Goodexam67:online}. However, the NLUs should be trained on more entities at different locations in the queries when using the prediction feature \cite{RASA_ner_crf_Features_code,Goodexam67:online}. 
%
%Finally, we highly recommend bot developers to use queries that are asked by real users to train the NLU when their bot is in production. Because it is difficult to include all the possible ways that users might ask the bot and entities, especially when it is deployed for the first time.

\begin{table*}[tbh]
	\caption{Recommendations for fine-tuning the NLUs when developing Chatbots.}
	\label{tab:recommendations}
	
	\begin{tabularx}{\linewidth}{llX}
		\toprule
		Problem & Recommendation \\
		\midrule
		\multirow{3}{*}{Low accuracy on intents classification} 
		& R1. Train NLUs with at least 10 queries per intent	\\
		& R2. Merge intents with similar words and disambiguate with a follow-up action				\\
%		& R3. Check the difference between in the confidence score in the top returned intents \\
		%\midrule
		& R3. Combine extra measures (e.g. regex, entity type) to aid to the confidence score \\
		%& R5. Fine-tune the confidence score threshold using the training set  \\
		
		\midrule
		
		\multirow{2}{*}{Low accuracy on entity extraction}
		& R4. Use different entity features (list feature vs prediction feature) according to the entity type \\
%		& R6. When using list feature, include as many synonims as possible\\
		& R5. When using entity prediction, focus on including entities in different query positions \\
		
		
		\bottomrule
	\end{tabularx}

\end{table*}
%Based on the findings of our study, we provide a set of recommendations to help developers and researchers to improve the performance of their NLU. 
%While our results are based on SE tasks, some of the guidelines can be used to improve  the NLU performance regardless of the domain, and increase their user's satisfaction. 
%We summarize all our recommendations in Table~\ref{tab:recommendations}, and discuss them in details in the following.
Based on our findings and experience in conducting this study, we provide a set of actionable recommendations to help chatbot practitioners to improve the performance of the used NLU. %Hence, increase the user's satisfaction~\cite{Naturall58:online,artifici16:online}.
Table~\ref{tab:recommendations} summarize our recommendations to improve the NLUs' performance in intents classifications and entity extraction.
While our results are based on SE tasks, some of the guidelines can be used to improve the NLU performance regardless of the domain. 
We discuss the recommendations in details in the following. 
\\

\noindent\textbf{R1. Train NLUs with at least 10 queries per intent.}
Our results show that the NLUs perform better when classifying queries with intents that have more training examples. 
While more data is typically better in any machine-learning task, the focus on crafting a good training set needs to be put in the diversity of queries per intent. 
Chatbot practitioners need to train the NLUs on at the very least 10 examples that represent different ways of querying a particular intent (e.g., having different sentence length~\cite{multiple17:online}). 
NLUs like Dialogflow and LUIS store the user input and the extracted intent~\cite{HistoryD17:online} and allow them to be retrained easily by confirming the extracted intent or labelled the queries with the correct intent. 
Chatbot developers should leverage this feature especially at the early stages of the chatbot development, as a part of the debugging process of the NLU and as a way of fine tuning the initial training set of the chatbot.
\\

\noindent\textbf{R2. Merge intents with similar words and disambiguate with a follow-up action.}
%Our results show that NLUs struggle in disambiguating intents that share a high number of common words and entity types. 
%Hence, it is worth to explore the possibility of merging such intents and program the chatbot to disambiguate such intents by asking a follow-up question. For example, if there is a chatbot that does code refactoring, then refactoring class or method intents have very similar training examples. In this case, the chatbot could ask the user back whether s/he would refactor a class or a method (if the name is not provided). 
%Merging intents also may increase the NLU intent classification accuracy by increasing the number of training examples for the merged intent.
The results show that NLUs better classify intents that contain exclusive words and distinct entity types, not shared with other intents.
Hence, it is worth exploring the possibility of merging intents that share a high number of common words and entity types and program the chatbot to disambiguate such intents by asking a follow-up question. For example, if there is a chatbot that does code refactoring, then refactoring class or method intents have very similar training examples. In this case, the chatbot could ask the user back whether s/he would refactor a class or a method (if the name is not provided). 
Merging intents also may increase the NLU intent classification accuracy by increasing the number of training examples for the merged intent.
\\

\noindent\textbf{R3. Combine other measures to aid the confidence score.}
%While most of the NLUs return high confidence scores when correctly classifying intents, as we discussed in Section~\ref{subsec:entityExtractionResult}, we recommend the chatbot developers use other measures to aid to the confidence score and improve the chatbot accuracy. For example, one measure that can be used by chatbot developers in case of all queries in the training set for a particular intent include a specific entity type is to verify the existence of an entity of that type in the query (e.g., queries of `FixingCommitsForBugTicket' intent has `JiraTicket' entity only).
While most of the NLUs return high confidence scores when correctly classifying intents, as we discussed in Section~\ref{subsec:entityExtractionResult}, we recommend the chatbot developers to use other measures to ensure the intent was classified correctly. For example, if an intent has a distinct entity type, then developers can check whether an entity of that type exists in the query and use that information to make sure that the intent was correctly classified (e.g., queries of `\BuggyCommit' intent has `JiraTicket' entity only).
\\

%For example, one measure that can be used by chatbot developers in case of all queries in the training set for a particular intent include a specific entity type is to verify the existence of an entity of that type in the query (e.g., queries of `\BuggyCommit' intent has `JiraTicket' entity only).



% Exploiting different entity features (list feature vs prediction feature)
\noindent\textbf{R4. Use different entity features according to the entity type.}
Developers should resort to different entity features (either list feature or prediction feature) together in the same chatbot, depending on the entities of their domain. 
Entities that are enumerable (e.g., months of the year) and have known finite values are better identified with the features containing all known synonims.
We observe this when evaluating the performance of entity extraction in the Repository task, where NLUs extracted entities more frequently corrected.
In most cases, however, an entity could be expressed in a variety of different (and unknown) ways and developers need to resort to prediction features. 
\\

%However, if an entity has an unknown synonims and can be expressed in different ways, developers need to resort to prediction features essentially. 

%The chatbot developers can use different features (list and prediction) together on the same chatbot. In other words, there are no restrictions to use one feature to extract entities from the user input. Developers can use the list feature when the entities and their synonyms are limited (e.g., commit hash). On the other hand, if the entities have a wide variety of words that make them difficult to define (e.g., programming languages), then using the prediction feature is the best.

% If using list feature - consider adding as many synonims as possible
%\noindent\textbf{R6. When using feature list, include as many synonims as possible.}
%The power of extracting entities using the list feature is proportional to the size of synonims list. For example, the `HHH846', `HHH-846', and `HHH 846' related to the `JiraTicket' entity. The developers need to take this into their consideration by training the NLUs on all ways in order to improve their extraction results~\cite{EntityIntentExtractionIBMWatson_link,Goodexam67:online}.

% When using entity prediction - consider training the NLU with entities in different position and part of speech
\noindent\textbf{R5. When using entity prediction feature, focus on including entities in different query positions.}
When it comes to extracting entities using the prediction feature, developers need to maximize the diversity in which the entities appear in their queries. 
An ideal training set should contain entities appearing in the beginning, middle and end of the queries to improve the NLU's ability of recognizing the entity in different contexts \cite{RASA_ner_crf_Features_code,Goodexam67:online}. 

%Table~\ref{tab:recommendations} summarize our recommendations to improve the NLUs' performance in intents classifications and entity extraction.


%\noindent\textbf{Ensemble NLUs for optimal performance}
%Researchers that need to reach an optimal performance should consider using multiple NLUs with a voting system to reach the optimal performance. Specifically, they can train and test multiple NLUs on the same dataset, record the NLUs' classification results for each query, and select the result returned by the majority of the leveraged NLUs as the final query's classification. This allows practitioners to minimize the shortcomings of specific NLUs by getting the best of all models.  Also, one could use such a system to label large datasets with a higher accuracy, by only training these models with just a small sample.
